ASVLite: a high-performance simulator for autonomous surface vehicles

The energy of ocean waves is the key distinguishing factor of marine environments compared to other aquatic environments such as lakes and rivers. Waves significantly affect the dynamics of marine vehicles; hence it is imperative to consider the dynamics of vehicles in waves when developing efficient control strategies for autonomous surface vehicles (ASVs). However, most marine simulators available open-source either exclude dynamics of vehicles in waves or use methods with high computational overhead. This paper presents ASVLite, a computationally efficient ASV simulator that uses frequency domain analysis for wave force computation. ASVLite is suitable for applications requiring low computational overhead and high run-time performance. Our tests on a Raspberry Pi 2 and a mid-range desktop computer show that the simulator has a high run-time performance to efficiently simulate irregular waves with a component wave count of up to 260 and large-scale swarms of up to 500 ASVs.

==> makefile <==
# A simple makefile to compile the tex files to a pdf document.
# Build targets provided:
# -----------------------
# make        : default compile option is make quiet.
# make quiet  : compile the tex files to pdf with minimal output message.
# make verbose: compile with detailed output messages.
# make view   : compile, if required, and view pdf file. 
# make clean  : clean all build files.

# Name of output pdf file
TARGET := IROS_2020

# Name of main tex file which includes all the other tex files.
MAIN := root

# Set the source and build directory
SRC_DIRS := ./
BUILD_DIR := ./build

# Collect all tex files and bib files.
SRCS := $(wildcard *.tex) \
        $(wildcard *.bib)

# Get versions of pdflatex and bibtex. This will be used to check if these applications exist.
PDFLATEX_VERSION := $(shell pdflatex --version 2>/dev/null)
BIBTEX_VERSION := $(shell bibtex --version 2>/dev/null)
# Check if all dependencies installed
ifdef PDFLATEX_VERSION
	ifdef BIBTEX_VERSION
		DEPENDENCIES_INSTALLED := 'true'
	endif
endif

# Compile the tex files
# ---------------------
# Each line of the build script has the following structure:
# -@command > /dev/null 2>&1 || true
# -           : to ignore the exit status of the command that is executed
#               and continue even if error encountered.
# @           : to suppresses the 'echo' of the command that is executed.
# > /dev/null : to redirect output (1) to /dev/null
# 2>&1        : to redirect error (2) to /dev/null 
# || true     : to suppress the "make: error ....(ignored)" output message.
#
# The last part '> /dev/null 2>&1 || true' is to make the output quiet

# Quiet compile
quiet: QUIET := > /dev/null 2>&1 || true
quiet: $(BUILD_DIR)/$(TARGET).pdf

# Verbous compile
verbose: QUIET := 
verbose: $(BUILD_DIR)/$(TARGET).pdf

# View the pdf 
# quiet is the build option for view
view: QUIET := > /dev/null 2>&1 || true
view: $(BUILD_DIR)/$(TARGET).pdf
	-@xdg-open $(BUILD_DIR)/$(TARGET).pdf > /dev/null 2>&1 || true &

# Compile pdf 
$(BUILD_DIR)/$(TARGET).pdf: $(SRCS)
	-@echo "--> Checking if pdflatex and bibtex are installed"
ifdef PDFLATEX_VERSION 
	-@echo "    --> pdflatex found."
else
	-@echo "    --> pdflatex not found."
endif
ifdef BIBTEX_VERSION 
	-@echo "    --> bibtex found."
else
	-@echo "    --> bibtex not found."
endif
# Proceed with compiling only if pdflatex and bibtex are found
ifdef DEPENDENCIES_INSTALLED
	-@echo "--> Making build directory if it does not exist"
	-@mkdir $(BUILD_DIR) $(QUIET)

	-@echo "--> pdflatex first run"
	-@pdflatex -interaction=nonstopmode -output-directory=$(BUILD_DIR) $(MAIN).tex $(QUIET)
	
	-@echo "--> run bibtex"
	-@bibtex $(BUILD_DIR)/$(MAIN) $(QUIET)
	
	-@echo "--> pdflatex second run"
	-@pdflatex -interaction=nonstopmode -output-directory=$(BUILD_DIR) $(MAIN).tex $(QUIET)
	
	-@echo "--> pdflatex final run"
	-@pdflatex -interaction=nonstopmode -output-directory=$(BUILD_DIR) $(MAIN).tex $(QUIET)
# Rename MAIN.pdf to TARGET.pdf if MAIN not equal to TARGET
ifneq ($(MAIN), $(TARGET)) 
	-@mv $(BUILD_DIR)/$(MAIN).pdf $(BUILD_DIR)/$(TARGET).pdf $(QUIET)
endif
# Check if the pdf file created. 
ifneq ("$(BUILD_DIR)/$(wildcard *.pdf)","")
	-@echo "--> Created $(BUILD_DIR)/$(TARGET).pdf"
else
	-@echo "--> Build failed possibly due to missing latex packages."
endif
# Else statement for: ifdef DEPENDENCIES_INSTALLED
else
	-@echo "--> Missing dependencies. Cannot compile."
endif

# Clean the build directory
.PHONY: clean
clean:
	-@$(RM) -r $(BUILD_DIR)
	-@echo "--> Build directory removed"

